The economic effects of nonlinear health dynamics: estimates from a dynamic life-cycle model

We study how nonlinear, state-dependent health dynamics shape economic behavior, inequality, and the evaluation of disability insurance at older ages. Using English panel data, we construct a continuous health index and estimate its dynamics with a flexible quantile-based method that allows persistence to vary across health states. We find that adverse health realizations are both larger and more persistent among individuals in poor health. Embedding the estimated process into a life-cycle model, we show that these state-dependent nonlinearities generate substantial losses in assets and welfare for economically vulnerable individuals-those with poor health and low wealth. Misspecifying health dynamics as state-independent attenuates these losses and leads to distorted savings behavior, with effects concentrated among vulnerable individuals. Finally, we find that the welfare losses of removing disability insurance are highly heterogeneous across health types, and are overstated by a state-independent health process.

==> images-IERrev/CompAggLHW.tex <==

Nonlinear   &       72289&      12.715&       0.578&       0.284\\
Linear      &       -6715&      -0.049&      -0.035&       0.030\\
Normal      &       -8211&      -0.077&      -0.054&       0.055\\
Linear--Estimated&        -497&      -0.042&      -0.036&       0.028\\


==> images-IERrev/CompAggZ1.tex <==

Nonlinear   &      104694&      12.606&       0.479&       0.210\\
Linear      &       -5293&      -0.046&      -0.032&       0.022\\
Normal      &       -6862&      -0.074&      -0.048&       0.044\\
Linear--Estimated&        1305&      -0.044&      -0.030&       0.009\\


==> images-IERrev/CompIn.tex <==

Nonlinear   &       54212&       0.481&       0.436&       0.035\\
Linear      &         532&       0.016&       0.009&       0.001\\
Normal      &         411&       0.023&       0.018&       0.002\\
Linear--Estimated&        1525&      -0.009&       0.002&       0.000\\


==> images-IERrev/CompInLH.tex <==

Nonlinear   &       49563&       0.527&       0.549&       0.044\\
Linear      &       -1151&       0.023&      -0.008&      -0.000\\
Normal      &       -1198&       0.030&       0.009&       0.001\\
Linear--Estimated&        -929&      -0.008&      -0.024&      -0.002\\


==> images-IERrev/dec_all_lin-bas.tex <==
None(baseline)      &      110001&       54743&        0.50&        0.72&        0.27&        0.18&           .\\
All (relative to baseline)&       30837&       -4108&       -0.14&        0.15&        0.27&       -0.15&       15.35\\
Mortality           &       -4576&          18&        0.02&       -0.01&       -0.02&        0.00&        9.03\\
Time cost           &       35577&       -3288&       -0.14&        0.14&        0.24&       -0.08&        7.06\\
Earnings            &        1199&         609&        0.00&        0.00&        0.00&        0.00&        0.23\\
DI                  &         906&       -1145&       -0.01&        0.05&        0.04&       -0.12&       -1.11\\


==> images-IERrev/dec_all_lno-bas.tex <==
None(baseline)      &      108203&       54623&        0.50&        0.71&        0.25&        0.19&           .\\
All (relative to baseline)&       32606&       -4111&       -0.15&        0.16&        0.29&       -0.16&       15.49\\
Mortality           &       -4615&         -28&        0.02&       -0.02&       -0.02&        0.00&        9.05\\
Time cost           &       36829&       -3496&       -0.15&        0.14&        0.25&       -0.09&        7.23\\
Earnings            &        1170&         624&        0.00&        0.00&        0.00&        0.00&        0.23\\
DI                  &         808&       -1120&       -0.01&        0.05&        0.05&       -0.13&       -1.23\\


==> images-IERrev/dec_earn_sd_top2_abb-bas.tex <==
None(baseline)      &        0.26&        0.40&        0.48&        0.54&        0.55&       12.47\\
All (relative to baseline)&       -0.06&       -0.10&       -0.18&       -0.18&       -0.15&        0.31\\


==> images-IERrev/dec_earn_sd_top2_lno-bas.tex <==
None(baseline)      &        0.25&        0.41&        0.50&        0.55&        0.56&       12.42\\
All (relative to baseline)&       -0.05&       -0.10&       -0.20&       -0.20&       -0.16&        0.36\\


==> images-IERrev/dec_earnings_sd_lin-bas.tex <==
None(baseline)      &        0.26&        0.41&        0.49&        0.55&        0.55&       12.44\\
All (relative to baseline)&       -0.06&       -0.10&       -0.19&       -0.19&       -0.16&        0.33\\
Mortality           &        0.00&        0.01&        0.01&        0.01&        0.01&       -0.02\\
Time cost           &       -0.06&       -0.09&       -0.15&       -0.13&       -0.11&        0.28\\
Earnings            &       -0.00&        0.00&        0.00&        0.00&        0.00&        0.01\\
DI                  &       -0.01&       -0.05&       -0.08&       -0.08&       -0.07&        0.10\\


==> images-IERrev/dec_earnings_sd_lno-bas.tex <==
None(baseline)      &        0.25&        0.41&        0.50&        0.55&        0.56&       12.42\\
All (relative to baseline)&       -0.05&       -0.10&       -0.20&       -0.20&       -0.16&        0.36\\
Mortality           &        0.00&        0.01&        0.01&        0.01&        0.01&       -0.03\\
Time cost           &       -0.05&       -0.09&       -0.15&       -0.13&       -0.11&        0.29\\
Earnings            &       -0.00&        0.00&        0.00&        0.00&        0.00&        0.01\\
DI                  &       -0.01&       -0.05&       -0.07&       -0.08&       -0.07&        0.11\\


==> images-IERrev/dec_top2_abb-bas.tex <==
None(baseline)      &      112618&       54212&        0.48&        0.73&        0.29&        0.16&           .\\
All (relative to baseline)&       28205&       -3603&       -0.12&        0.14&        0.25&       -0.14&       15.05\\


==> images-IERrev/dec_top2_lno-bas.tex <==
None(baseline)      &      108203&       54623&        0.50&        0.71&        0.25&        0.19&           .\\
All (relative to baseline)&       32606&       -4111&       -0.15&        0.16&        0.29&       -0.16&       15.49\\


==> images-IERrev/earncostZeta_nbs.tex <==
Baseline            &         932&        2256&        4425&         865&        1897&        3338&         577&        1450&        2678\\
Linear              &         676&        2048&        4315&         827&        1914&        3491&         575&        1535&        2885\\
\linreest           &         654&        1958&        3856&         817&        1862&        3289&         554&        1513&        2774\\


==> images-IERrev/earncost_nbs.tex <==
Baseline            &         692&        1749&        3264\\
Linear              &         636&        1741&        3336\\
\linreest           &         623&        1699&        3146\\


==> images-IERrev/incomecostZeta_nbs.tex <==
Baseline            &           0&        1536&        3247&         319&        1368&        2525&         265&        1045&        2047\\
Linear              &           0&        1362&        3240&         208&        1355&        2696&         229&        1092&        2219\\
\linreest           &           0&        1337&        2979&         243&        1338&        2538&         236&        1094&        2150\\


==> images-IERrev/incomecost_nbs.tex <==
Baseline            &         218&        1226&        2454\\
Linear              &         113&        1212&        2545\\
\linreest           &         139&        1204&        2420\\


==> images-IERrev/nodi_welfare.tex <==
Baseline            &       -1.17&       -0.65&       -0.37\\
Linear              &       -1.63&       -0.69&       -0.35\\
\linreest           &       -1.69&       -0.70&       -0.35\\


==> images-IERrev/nodi_welfare_byh.tex <==
Baseline            &       -4.92&       -2.34&       -1.06&       -0.47\\
Linear              &       -5.22&       -2.38&       -1.32&       -0.44\\
\linreest           &       -6.53&       -2.55&       -1.38&       -0.44\\


==> images-IERrev/nodi_welfare_revneu.tex <==
Baseline            &        2.65&        4.18&        5.45\\
Linear              &        2.64&        4.43&        5.78\\
\linreest           &        2.56&        4.44&        5.78\\


==> images-IERrev/nodi_welfare_revneu_byh.tex <==
Baseline            &        1.95&        3.73&        4.43&        4.28\\
Linear              &        1.97&        3.85&        4.56&        4.58\\
\linreest           &        0.74&        3.71&        4.54&        4.64\\


==> images-IERrev/welfareZeta_nbs.tex <==
Baseline            &        1808&        2902&        5115&        1643&        2446&        4078&        1233&        2004&        3434\\
Linear              &        1592&        2791&        5131&        1627&        2587&        4403&        1244&        2159&        3838\\
\linreest           &        1587&        2862&        5187&        1678&        2694&        4526&        1254&        2255&        3941\\


==> images-IERrev/welfare_nbs.tex <==
Baseline            &        1417&        2346&        4107\\
Linear              &        1394&        2425&        4334\\
\linreest           &        1411&        2503&        4410\\


==> images-IERrev/welfareshocksZ_10_11.tex <==
scaleCC11           &         -14&         925&         221&        1271&         511&        1847\\
scaleCC11           &          76&         352&         108&         514&         136&         648\\


==> images-IERrev/welfareshocksZ_10_21.tex <==
scaleCC21           &         361&         947&         455&        1060&         445&        1096\\
scaleCC21           &         147&         617&         193&         726&         193&         755\\


==> images-IERrev/welfareshocksZ_80_11.tex <==
scaleCC11           &        -283&         535&        -433&         664&         -80&        1238\\
scaleCC11           &          61&         330&          73&         514&         113&         636\\


==> images-IERrev/welfareshocksZ_nodi_10_11.tex <==
Nonlinear(baseline) &         926&        2728&        1354&        3215&        1606&        3724\\
Linear (same likelihood shocks)&         189&         676&         199&         775&         225&         835\\


==> images-IERrev/welfareshocksZ_nodi_10_21.tex <==
Nonlinear(baseline) &         509&        1222&         549&        1269&         495&        1269\\
Linear (same likelihood shocks)&         204&         766&         226&         821&         206&         829\\


==> images-IERrev/welfareshocksZ_nodi_80_11.tex <==
Nonlinear(baseline) &         653&        2309&         872&        2692&        1115&        3099\\
Linear (same likelihood shocks)&         158&         631&         151&         680&         174&         725\\


==> images-IERrev/welfareshocks_10_11.tex <==
Nonlinear(baseline) &         284&        1492\\
Linear (same likelihood shocks)&         107&         531\\


==> images-IERrev/welfareshocks_10_21.tex <==
Nonlinear(baseline) &         421&        1047\\
Linear (same likelihood shocks)&         178&         710\\


==> images-IERrev/welfareshocks_80_11.tex <==
Nonlinear(baseline) &        -207&         872\\
Linear (same likelihood shocks)&          86&         513\\


==> images-IERrev/welfareshocks_allA_10_11.tex <==
Nonlinear(baseline) &        -669&         284&        1492&        -143&        1351&        3356\\
Linear (same likelihood shocks)&        -280&         107&         531&        -283&         206&         779\\


==> images-IERrev/welfareshocks_allA_10_21.tex <==
Nonlinear(baseline) &        -100&         421&        1047&         -51&         511&        1254\\
Linear (same likelihood shocks)&        -268&         178&         710&        -290&         209&         806\\


==> images-IERrev/welfareshocks_allA_80_11.tex <==
Nonlinear(baseline) &       -1504&        -207&         872&        -226&         928&        2774\\
Linear (same likelihood shocks)&        -403&          86&         513&        -277&         163&         684\\


==> images-IERrev/welfareshocks_nodi_10_11.tex <==
Nonlinear(baseline) &        1351&        3356\\
Linear (same likelihood shocks)&         206&         779\\


==> images-IERrev/welfareshocks_nodi_10_21.tex <==
Nonlinear(baseline) &         511&        1254\\
Linear (same likelihood shocks)&         209&         806\\


==> images-IERrev/welfareshocks_nodi_80_11.tex <==
Nonlinear(baseline) &         928&        2774\\
Linear (same likelihood shocks)&         163&         684\\


==> images/CompAgg.tex <==
            % &      Assets&    Earnings&        Work&     DI rate\\
%  \textbf {All} &&&& \\ \hline
            Nonlinear   &      112618&      12.661&       0.518&       0.162\\
Linear      &       -2617&      -0.022&      -0.016&       0.014\\
Normal      &       -4415&      -0.043&      -0.030&       0.026\\
Linear--Estimated&        5417&      -0.018&      -0.013&       0.004\\


==> images/CompAggLH.tex <==
 %           &      Assets&    Earnings&        Work&     DI rate\\

Nonlinear   &       94012&      12.636&       0.471&       0.319\\
Linear      &       -6014&      -0.052&      -0.032&       0.025\\
Normal      &       -7185&      -0.083&      -0.050&       0.053\\
Linear--Estimated&        -342&      -0.049&      -0.031&       0.012\\


==> images/CompAggLHW.tex <==
          %  &      Assets&    Earnings&        Work&     DI rate\\
%\textbf {Low health and wealth} &&&& \\ \hline

Nonlinear   &       72289&      12.715&       0.578&       0.284\\
Linear      &       -6715&      -0.049&      -0.035&       0.030\\
Normal      &       -8211&      -0.077&      -0.054&       0.055\\
Linear--Estimated&        -497&      -0.042&      -0.036&       0.028\\


==> images/dec_all_abb-bas.tex <==
None (baseline)      &      112618&       54212&        0.48&        0.73&        0.29&        0.16&           .\\
All (relative to baseline) &       28205&       -3603&       -0.12&        0.14&        0.25&       -0.14&       11.32\\
Mortality           &       -4779&         -30&        0.02&       -0.01&       -0.02&        0.00&        5.00\\
Time cost           &       34037&       -1763&       -0.12&        0.12&        0.22&       -0.07&        6.96\\
Earnings            &         905&         505&        0.00&        0.00&        0.00&        0.00&        0.17\\
DI                  &         759&        -632&       -0.01&        0.05&        0.04&       -0.11&       -0.95\\


==> images/dec_earn_sd_top2_lin-bas.tex <==
None(baseline)      &        0.26&        0.41&        0.49&        0.55&        0.55&       12.44\\
All (relative to baseline)&       -0.06&       -0.10&       -0.19&       -0.19&       -0.16&        0.33\\


==> images/dec_earn_sd_top2_lll-bas.tex <==
None(baseline)      &        0.26&        0.40&        0.48&        0.53&        0.55&       12.45\\
All (relative to baseline)&       -0.08&       -0.13&       -0.20&       -0.19&       -0.15&        0.33\\


==> images/dec_earn_sd_top2_lno-bas.tex <==
None(baseline)      &        0.25&        0.41&        0.50&        0.55&        0.56&       12.42\\
All (relative to baseline)&       -0.05&       -0.10&       -0.20&       -0.20&       -0.16&        0.36\\


==> images/dec_earnings_sd_abb-bas.tex <==
None(baseline)      &        0.26&        0.40&        0.48&        0.54&        0.55&       12.47\\
All (relative to baseline)&       -0.06&       -0.10&       -0.18&       -0.18&       -0.15&        0.31\\
Mortality           &        0.00&        0.01&        0.01&        0.00&        0.00&       -0.02\\
Time cost           &       -0.05&       -0.08&       -0.14&       -0.13&       -0.11&        0.26\\
Earnings            &       -0.00&        0.00&        0.01&        0.01&        0.01&        0.01\\
DI                  &       -0.01&       -0.04&       -0.07&       -0.07&       -0.06&        0.09\\


==> images/dec_top2_lin-bas.tex <==
None(baseline)      &      110001&       54743&        0.50&        0.72&        0.27&        0.18&           .\\
All (relative to baseline)&       30837&       -4108&       -0.14&        0.15&        0.27&       -0.15&       11.64\\


==> images/dec_top2_lll-bas.tex <==
None(baseline)      &      118034&       55737&        0.47&        0.72&        0.27&        0.17&           .\\
All (relative to baseline)&       32623&       -5748&       -0.14&        0.15&        0.26&       -0.14&       12.10\\


==> images/dec_top2_lno-bas.tex <==
None(baseline)      &      108203&       54623&        0.50&        0.71&        0.25&        0.19&           .\\
All (relative to baseline)&       32606&       -4111&       -0.15&        0.16&        0.29&       -0.16&       11.80\\


==> images/earnings_table_old.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
            &\multicolumn{1}{c}{wpactive}&\multicolumn{1}{c}{deltalogw}&\multicolumn{1}{c}{logw}\\
\hline
            &                     &                     &                     \\
age         &       0.101         &     0.059           &       0.465\sym{***}\\
            &     (0.084)         &    (0.144)          &     (0.059)         \\
[1em]
age2        &      -0.002\sym{*}  &    -0.001           &      -0.004\sym{***}\\
            &     (0.001)         &    (0.001)          &     (0.001)         \\
[1em]
Hindex      &       0.304\sym{***}&     0.007           &       0.097\sym{**} \\
            &     (0.048)         &    (0.049)          &     (0.034)         \\
[1em]
Hindex2     &      -0.138\sym{***}&     0.092           &       0.046\sym{*}  \\
            &     (0.035)         &    (0.048)          &     (0.023)         \\
[1em]
Hindex3     &       0.007         &    -0.042           &      -0.007         \\
            &     (0.029)         &    (0.025)          &     (0.021)         \\
[1em]
Hindex4     &       0.001         &    -0.019           &      -0.008         \\
            &     (0.009)         &    (0.013)          &     (0.005)         \\
% [1em]
% couple      &      -0.099         &                     &      -0.571\sym{*}  \\
%             &     (0.768)         &                     &     (0.290)         \\
% [1em]
% yrd1        &      -0.274\sym{***}&                     &      -0.068         \\
%             &     (0.059)         &                     &     (0.050)         \\
% [1em]
% yrd2        &      -0.247\sym{***}&                     &      -0.087         \\
%             &     (0.059)         &                     &     (0.051)         \\
% [1em]
% yrd3        &      -0.176\sym{**} &                     &      -0.011         \\
%             &     (0.062)         &                     &     (0.053)         \\
% [1em]
% yrd4        &      -0.067         &                     &      -0.025         \\
%             &     (0.054)         &                     &     (0.048)         \\
% [1em]
% yrd5        &      -0.072         &                     &      -0.026         \\
%             &     (0.051)         &                     &     (0.048)         \\
% [1em]
% yrd6        &      -0.071         &                     &      -0.050         \\
%             &     (0.046)         &                     &     (0.046)         \\
% [1em]
% yrd7        &      -0.044         &                     &      -0.060         \\
%             &     (0.039)         &                     &     (0.045)         \\
% [1em]
% yrd8        &       0.000         &                     &       0.000         \\
%             &         (.)         &                     &         (.)         \\
% [1em]
% 0.childyoung&       0.000         &                     &                     \\
%             &         (.)         &                     &                     \\
% [1em]
% 1.childyoung&       0.184\sym{***}&                     &                     \\
%             &     (0.047)         &                     &                     \\
% [1em]
% 0.spage     &       0.000         &                     &                     \\
%             &         (.)         &                     &                     \\
% [1em]
% 1.spage     &      -0.286\sym{***}&                     &                     \\
%             &     (0.046)         &                     &                     \\
% [1em]
% 0.spage\_p   &       0.000         &                     &                     \\
%             &         (.)         &                     &                     \\
% [1em]
% 1.spage\_p   &      -0.165\sym{***}&                     &                     \\
%             &     (0.043)         &                     &                     \\
% [1em]
% 0.healthpart&       0.000         &                     &                     \\
%             &         (.)         &                     &                     \\
% [1em]
% 1.healthpart&      -0.237\sym{***}&                     &                     \\
%             &     (0.047)         &                     &                     \\
% [1em]
% deltaage    &                     &       0.059         &                     \\
%             &                     &     (0.144)         &                     \\
% [1em]
% deltaage2   &                     &      -0.001         &                     \\
%             &                     &     (0.001)         &                     \\
% [1em]
% deltaHindex &                     &       0.007         &                     \\
%             &                     &     (0.049)         &                     \\
% [1em]
% deltaHindex2&                     &       0.092         &                     \\
%             &                     &     (0.048)         &                     \\
% [1em]
% deltaHindex3&                     &      -0.042         &                     \\
%             &                     &     (0.025)         &                     \\
% [1em]
% deltaHindex4&                     &      -0.019         &                     \\
%             &                     &     (0.013)         &                     \\
% [1em]
% deltacouple &                     &      -0.282         &                     \\
%             &                     &     (0.302)         &                     \\
% [1em]
% deltayrd1   &                     &       0.000         &                     \\
%             &                     &         (.)         &                     \\
% [1em]
% deltayrd2   &                     &       0.032         &                     \\
%             &                     &     (0.154)         &                     \\
% [1em]
% deltayrd3   &                     &       0.073         &                     \\
%             &                     &     (0.293)         &                     \\
% [1em]
% deltayrd4   &                     &      -0.020         &                     \\
%             &                     &     (0.439)         &                     \\
% [1em]
% deltayrd5   &                     &      -0.034         &                     \\
%             &                     &     (0.583)         &                     \\
% [1em]
% deltayrd6   &                     &      -0.067         &                     \\
%             &                     &     (0.725)         &                     \\
% [1em]
% deltayrd7   &                     &      -0.082         &                     \\
%             &                     &     (0.871)         &                     \\
% [1em]
% deltayrd8   &                     &      -0.043         &                     \\
%             &                     &     (1.018)         &                     \\
% [1em]
% lamda0      &                     &      -0.368         &                     \\
%             &                     &     (0.210)         &                     \\
% [1em]
% \_IgapXlamd\_4&                     &      -0.389         &                     \\
%             &                     &     (0.330)         &                     \\
% [1em]
% \_IgapXlamd\_6&                     &       2.214\sym{***}&                     \\
%             &                     &     (0.505)         &                     \\
% [1em]
% \_IgapXlamd\_8&                     &      -2.537         &                     \\
%             &                     &     (2.782)         &                     \\
% [1em]
% \_IgapXlamd\_10&                     &       0.000         &                     \\
%             &                     &         (.)         &                     \\
% [1em]
% \_IgapXlamd\_12&                     &       0.000         &                     \\
%             &                     &         (.)         &                     \\
% [1em]
% lag1lamda0  &                     &       0.346         &                     \\
%             &                     &     (0.237)         &                     \\
% [1em]
% \_IgapXlag1\_4&                     &       0.397         &                     \\
%             &                     &     (0.436)         &                     \\
% [1em]
% \_IgapXlag1\_6&                     &      -6.001\sym{***}&                     \\
%             &                     &     (1.395)         &                     \\
% [1em]
% \_IgapXlag1\_8&                     &       9.749         &                     \\
%             &                     &     (7.019)         &                     \\
% [1em]
% \_IgapXlag1\_10&                     &       0.000         &                     \\
%             &                     &         (.)         &                     \\
% [1em]
% \_IgapXlag1\_12&                     &       0.000         &                     \\
%             &                     &         (.)         &                     \\
% [1em]
% \_cons      &       1.112         &       0.018         &      -1.921         \\
%             &     (2.618)         &     (0.119)         &     (1.728)         \\
\hline
N observations&       14171         &        4238         &        6505         \\
p-value excl. restr.&       0.000   &                     &                     \\
p-value sel. corr.&                 &       0.001         &                     \\
p-value health&                     &       0.246         &       0.000         \\
\hline\hline
\multicolumn{4}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{4}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}


==> images/ineqdecompabb10.0.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
	\multirow{2}{*}{Effects removed} & 
	\multicolumn{4}{c}{\hspace{1em} Assets} &	 \multicolumn{4}{c}{\hspace{1em} Cum. earnings} \\
	 & \multicolumn{2}{r}{80/20pct}   & \multicolumn{2}{r}{Std.} & \multicolumn{2}{r}{80/20pct.}   & \multicolumn{2}{r}{Std. (log)} \\  
 \midrule 
	 None (Baseline)            
	 & \multicolumn{2}{c}{ \hspace{1em}3.41 }  
	 & \multicolumn{2}{c}{ \hspace{1em} 98 }  
	 & \multicolumn{2}{c}{ \hspace{1em}2.45 }  
	 & \multicolumn{2}{c}{ \hspace{1em}0.74 }   \\  
 \\ \multicolumn{9}{c}{(a) Counterfactual health: 10th  percentile} \\
	 All (relative to baseline) & +68&\% &  +1&\% &  -2&\% &  -3&\%  \\  
	 Decomposition: &&&&&&&& \\
	 \hspace{1em}Mortality      &  +5&\% &  +0&\% &  +1&\% &  +0&\%  \\  
	 \hspace{1em}Time cost      & +43 &  &  +1 &  &  -4 &  &  -4 &   \\  
	 \hspace{1em}Wages          &  +8 &  &  -0 &  &  -2 &  &  -2 &   \\  
	 \hspace{1em}Mortality+Time & +51 &  &  +1 &  &  -3 &  &  -3 &   \\  
	 \hspace{1em}Mortality+Wages& +14 &  &  +0 &  &  -0 &  &  -2 &   \\  
	 \hspace{1em}Time+Wages     & +64 &  &  +2 &  &  -3 &  &  -4 &   \\  
\bottomrule
\end{tabular}

==> images/ineqdecompabb25.0.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
	\multirow{2}{*}{Effects removed} & 
	\multicolumn{4}{c}{\hspace{1em} Assets} &	 \multicolumn{4}{c}{\hspace{1em} Cum. earnings} \\
	 & \multicolumn{2}{r}{80/20pct}   & \multicolumn{2}{r}{Std.} & \multicolumn{2}{r}{80/20pct.}   & \multicolumn{2}{r}{Std. (log)} \\  
 \midrule 
	 None (Baseline)            
	 & \multicolumn{2}{c}{ \hspace{1em}3.41 }  
	 & \multicolumn{2}{c}{ \hspace{1em} 98 }  
	 & \multicolumn{2}{c}{ \hspace{1em}2.45 }  
	 & \multicolumn{2}{c}{ \hspace{1em}0.74 }   \\  
 \\ \multicolumn{9}{c}{(a) Counterfactual health: 25th  percentile} \\
	 All (relative to baseline) & +35&\% &  +1&\% &  -9&\% &  -4&\%  \\  
	 Decomposition: &&&&&&&& \\
	 \hspace{1em}Mortality      &  +3&\% &  +0&\% &  -0&\% &  -0&\%  \\  
	 \hspace{1em}Time cost      & +23 &  &  +0 &  & -10 &  &  -5 &   \\  
	 \hspace{1em}Wages          &  +4 &  &  -0 &  &  -3 &  &  -3 &   \\  
	 \hspace{1em}Mortality+Time & +25 &  &  +0 &  & -10 &  &  -5 &   \\  
	 \hspace{1em}Mortality+Wages&  +5 &  &  -0 &  &  -3 &  &  -3 &   \\  
	 \hspace{1em}Time+Wages     & +33 &  &  +1 &  &  -9 &  &  -4 &   \\  
\bottomrule
\end{tabular}

==> images/ineqdecompabb75.0.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
	\multirow{2}{*}{Effects removed} & 
	\multicolumn{4}{c}{\hspace{1em} Assets} &	 \multicolumn{4}{c}{\hspace{1em} Cum. earnings} \\
	 & \multicolumn{2}{r}{80/20pct}   & \multicolumn{2}{r}{Std.} & \multicolumn{2}{r}{80/20pct.}   & \multicolumn{2}{r}{Std. (log)} \\  
 \midrule 
	 None (Baseline)            
	 & \multicolumn{2}{c}{ \hspace{1em}3.41 }  
	 & \multicolumn{2}{c}{ \hspace{1em} 98 }  
	 & \multicolumn{2}{c}{ \hspace{1em}2.45 }  
	 & \multicolumn{2}{c}{ \hspace{1em}0.74 }   \\  
 \\ \multicolumn{9}{c}{(a) Counterfactual health: 75th  percentile} \\
	 All (relative to baseline) & -28&\% &  -8&\% & -20&\% & -19&\%  \\  
	 Decomposition: &&&&&&&& \\
	 \hspace{1em}Mortality      &  +0&\% &  -0&\% &  -1&\% &  -1&\%  \\  
	 \hspace{1em}Time cost      & -25 &  &  -6 &  & -19 &  & -16 &   \\  
	 \hspace{1em}Wages          &  -6 &  &  -1 &  &  -4 &  &  -4 &   \\  
	 \hspace{1em}Mortality+Time & -26 &  &  -7 &  & -20 &  & -17 &   \\  
	 \hspace{1em}Mortality+Wages&  -6 &  &  -1 &  &  -5 &  &  -5 &   \\  
	 \hspace{1em}Time+Wages     & -27 &  &  -7 &  & -20 &  & -18 &   \\  
\bottomrule
\end{tabular}

==> images/ineqdecompabb90.0.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
	\multirow{2}{*}{Effects removed} & 
	\multicolumn{4}{c}{\hspace{1em} Assets} &	 \multicolumn{4}{c}{\hspace{1em} Cum. earnings} \\
	 & \multicolumn{2}{r}{80/20pct}   & \multicolumn{2}{r}{Std.} & \multicolumn{2}{r}{80/20pct.}   & \multicolumn{2}{r}{Std. (log)} \\  
 \midrule 
	 None (Baseline)            
	 & \multicolumn{2}{c}{ \hspace{1em}3.41 }  
	 & \multicolumn{2}{c}{ \hspace{1em} 98 }  
	 & \multicolumn{2}{c}{ \hspace{1em}2.45 }  
	 & \multicolumn{2}{c}{ \hspace{1em}0.74 }   \\  
 \\ \multicolumn{9}{c}{(a) Counterfactual health: 90th  percentile} \\
	 All (relative to baseline) & -34&\% &  -9&\% & -23&\% & -26&\%  \\  
	 Decomposition: &&&&&&&& \\
	 \hspace{1em}Mortality      &  -0&\% &  -0&\% &  -1&\% &  -1&\%  \\  
	 \hspace{1em}Time cost      & -29 &  &  -8 &  & -22 &  & -22 &   \\  
	 \hspace{1em}Wages          &  -7 &  &  -1 &  &  -5 &  &  -7 &   \\  
	 \hspace{1em}Mortality+Time & -31 &  &  -8 &  & -23 &  & -23 &   \\  
	 \hspace{1em}Mortality+Wages&  -7 &  &  -1 &  &  -6 &  &  -8 &   \\  
	 \hspace{1em}Time+Wages     & -31 &  &  -8 &  & -23 &  & -25 &   \\  
\bottomrule
\end{tabular}

==> images/ineqdecompabb9010.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
	\multirow{2}{*}{Effects removed} & 
	\multicolumn{4}{c}{\hspace{1em} Assets} &	 \multicolumn{4}{c}{\hspace{1em} Cum. earnings} \\
	 & \multicolumn{2}{r}{80/20pct}   & \multicolumn{2}{r}{Std.} & \multicolumn{2}{r}{80/20pct.}   & \multicolumn{2}{r}{Std. (log)} \\  
 \midrule 
	 None (Baseline)            
	 & \multicolumn{2}{c}{ \hspace{1em}3.41 }  
	 & \multicolumn{2}{c}{ \hspace{1em} 98 }  
	 & \multicolumn{2}{c}{ \hspace{1em}2.45 }  
	 & \multicolumn{2}{c}{ \hspace{1em}0.74 }   \\  
 \\ \multicolumn{9}{c}{(a) Counterfactual health: 90th  percentile} \\
	 All (relative to baseline) & -34&\% &  -9&\% & -23&\% & -26&\%  \\  
	 Decomposition: &&&&&&&& \\
	 \hspace{1em}Mortality      &  -0&\% &  -0&\% &  -1&\% &  -1&\%  \\  
	 \hspace{1em}Time cost      & -29 &  &  -8 &  & -22 &  & -22 &   \\  
	 \hspace{1em}Wages          &  -7 &  &  -1 &  &  -5 &  &  -7 &   \\  
	 \hspace{1em}Mortality+Time & -31 &  &  -8 &  & -23 &  & -23 &   \\  
	 \hspace{1em}Mortality+Wages&  -7 &  &  -1 &  &  -6 &  &  -8 &   \\  
	 \hspace{1em}Time+Wages     & -31 &  &  -8 &  & -23 &  & -25 &   \\  
 \\ \multicolumn{9}{c}{(b) Counterfactual health: 10th  percentile} \\
	 All (relative to baseline) & +68&\% &  +1&\% &  -2&\% &  -3&\%  \\ 
\bottomrule
\end{tabular}

==> images/ineqdecompar110.0.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
	\multirow{2}{*}{Effects removed} & 
	\multicolumn{4}{c}{\hspace{1em} Assets} &	 \multicolumn{4}{c}{\hspace{1em} Cum. earnings} \\
	 & \multicolumn{2}{r}{80/20pct}   & \multicolumn{2}{r}{Std.} & \multicolumn{2}{r}{80/20pct.}   & \multicolumn{2}{r}{Std. (log)} \\  
 \midrule 
	 None (Baseline)            
	 & \multicolumn{2}{c}{ \hspace{1em}3.26 }  
	 & \multicolumn{2}{c}{ \hspace{1em} 98 }  
	 & \multicolumn{2}{c}{ \hspace{1em}2.65 }  
	 & \multicolumn{2}{c}{ \hspace{1em}0.77 }   \\  
 \\ \multicolumn{9}{c}{(a) Counterfactual health: 10th  percentile} \\
	 All (relative to baseline) & +106&\% &  +2&\% & +19&\% &  +1&\%  \\  
	 Decomposition: &&&&&&&& \\
	 \hspace{1em}Mortality      &  +4&\% &  +1&\% &  +1&\% &  +0&\%  \\  
	 \hspace{1em}Time cost      & +65 &  &  +1 &  & +16 &  &  +1 &   \\  
	 \hspace{1em}Wages          & +10 &  &  -0 &  &  -3 &  &  -1 &   \\  
	 \hspace{1em}Mortality+Time & +68 &  &  +1 &  & +16 &  &  +0 &   \\  
	 \hspace{1em}Mortality+Wages& +12 &  &  +0 &  &  -1 &  &  -1 &   \\  
	 \hspace{1em}Time+Wages     & +96 &  &  +2 &  & +19 &  &  +1 &   \\  
\bottomrule
\end{tabular}

==> images/ineqdecompar125.0.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
	\multirow{2}{*}{Effects removed} & 
	\multicolumn{4}{c}{\hspace{1em} Assets} &	 \multicolumn{4}{c}{\hspace{1em} Cum. earnings} \\
	 & \multicolumn{2}{r}{80/20pct}   & \multicolumn{2}{r}{Std.} & \multicolumn{2}{r}{80/20pct.}   & \multicolumn{2}{r}{Std. (log)} \\  
 \midrule 
	 None (Baseline)            
	 & \multicolumn{2}{c}{ \hspace{1em}3.26 }  
	 & \multicolumn{2}{c}{ \hspace{1em} 98 }  
	 & \multicolumn{2}{c}{ \hspace{1em}2.65 }  
	 & \multicolumn{2}{c}{ \hspace{1em}0.77 }   \\  
 \\ \multicolumn{9}{c}{(a) Counterfactual health: 25th  percentile} \\
	 All (relative to baseline) &  +9&\% &  -1&\% & -15&\% &  -9&\%  \\  
	 Decomposition: &&&&&&&& \\
	 \hspace{1em}Mortality      &  +3&\% &  +0&\% &  -0&\% &  -0&\%  \\  
	 \hspace{1em}Time cost      &  -2 &  &  -1 &  & -14 &  & -10 &   \\  
	 \hspace{1em}Wages          &  +3 &  &  -1 &  &  -4 &  &  -2 &   \\  
	 \hspace{1em}Mortality+Time &  -0 &  &  -1 &  & -14 &  &  -9 &   \\  
	 \hspace{1em}Mortality+Wages&  +7 &  &  -1 &  &  -4 &  &  -2 &   \\  
	 \hspace{1em}Time+Wages     &  +9 &  &  -1 &  & -15 &  &  -9 &   \\  
\bottomrule
\end{tabular}

==> images/ineqdecompar175.0.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
	\multirow{2}{*}{Effects removed} & 
	\multicolumn{4}{c}{\hspace{1em} Assets} &	 \multicolumn{4}{c}{\hspace{1em} Cum. earnings} \\
	 & \multicolumn{2}{r}{80/20pct}   & \multicolumn{2}{r}{Std.} & \multicolumn{2}{r}{80/20pct.}   & \multicolumn{2}{r}{Std. (log)} \\  
 \midrule 
	 None (Baseline)            
	 & \multicolumn{2}{c}{ \hspace{1em}3.26 }  
	 & \multicolumn{2}{c}{ \hspace{1em} 98 }  
	 & \multicolumn{2}{c}{ \hspace{1em}2.65 }  
	 & \multicolumn{2}{c}{ \hspace{1em}0.77 }   \\  
 \\ \multicolumn{9}{c}{(a) Counterfactual health: 75th  percentile} \\
	 All (relative to baseline) & -24&\% &  -7&\% & -24&\% & -17&\%  \\  
	 Decomposition: &&&&&&&& \\
	 \hspace{1em}Mortality      &  -0&\% &  -0&\% &  -1&\% &  -1&\%  \\  
	 \hspace{1em}Time cost      & -19 &  &  -6 &  & -22 &  & -14 &   \\  
	 \hspace{1em}Wages          &  -7 &  &  -1 &  &  -7 &  &  -5 &   \\  
	 \hspace{1em}Mortality+Time & -21 &  &  -6 &  & -23 &  & -15 &   \\  
	 \hspace{1em}Mortality+Wages&  -7 &  &  -1 &  &  -8 &  &  -6 &   \\  
	 \hspace{1em}Time+Wages     & -22 &  &  -6 &  & -23 &  & -16 &   \\  
\bottomrule
\end{tabular}

==> images/ineqdecompar190.0.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
		 >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
	\multirow{2}{*}{Effects removed} & 
	\multicolumn{4}{c}{\hspace{1em} Assets} &	 \multicolumn{4}{c}{\hspace{1em} Cum. earnings} \\
	 & \multicolumn{2}{r}{80/20pct}   & \multicolumn{2}{r}{Std.} & \multicolumn{2}{r}{80/20pct.}   & \multicolumn{2}{r}{Std. (log)} \\  
 \midrule 
	 None (Baseline)            
	 & \multicolumn{2}{c}{ \hspace{1em}3.26 }  
	 & \multicolumn{2}{c}{ \hspace{1em} 98 }  
	 & \multicolumn{2}{c}{ \hspace{1em}2.65 }  
	 & \multicolumn{2}{c}{ \hspace{1em}0.77 }   \\  
 \\ \multicolumn{9}{c}{(a) Counterfactual health: 90th  percentile} \\
	 All (relative to baseline) & -29&\% &  -8&\% & -27&\% & -22&\%  \\  
	 Decomposition: &&&&&&&& \\
	 \hspace{1em}Mortality      &  -0&\% &  -0&\% &  -1&\% &  -1&\%  \\  
	 \hspace{1em}Time cost      & -23 &  &  -7 &  & -24 &  & -16 &   \\  
	 \hspace{1em}Wages          &  -8 &  &  -1 &  &  -9 &  &  -8 &   \\  
	 \hspace{1em}Mortality+Time & -26 &  &  -7 &  & -25 &  & -17 &   \\  
	 \hspace{1em}Mortality+Wages&  -9 &  &  -1 &  & -10 &  &  -8 &   \\  
	 \hspace{1em}Time+Wages     & -27 &  &  -7 &  & -26 &  & -21 &   \\  
\bottomrule
\end{tabular}

==> images/ineqtable.tex <==
\begin{tabular}[ht]{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Initial health/Variable}} & \multicolumn{6}{c}{\textbf{Model}} \\
\cmidrule(r){2-7}
 & \multicolumn{3}{c}{\textbf{Nonlinear}} &  \multicolumn{3}{c}{\textbf{Canonical}} \\
 & Std. & 80/50 & 50/20 & Std. & 80/50 & 50/20 \\
\midrule
\textbf{All} & & & \\
Assets ($\times 1,000$)  &    98 &  1.42 &  2.40 &    98 &  1.42 &  2.29 \\
Hours                    &   630 &  1.55 &  1.50 &   648 &  1.32 &  1.84 \\
Cum. earnings ($\times 1,000)$   &   121 &  1.44 &  1.75 &   127 &  1.47 &  1.92 \\
\midrule
\textbf{0-10} & & & \\
Assets ($\times 1,000$)  &    88 &  2.34 & 223.18 &    91 &  1.87 & 10.15 \\
Hours                    &   545 &  1.94 &  1.00 &   615 &  1.79 &  1.12 \\
Cum. earnings ($\times 1,000)$   &   111 &  1.68 &  2.52 &   114 &  1.73 &  2.65 \\
\midrule
\textbf{10-25} & & & \\
Assets ($\times 1,000$)  &   103 &  1.67 &  3.80 &   102 &  1.64 &  3.73 \\
Hours                    &   574 &  1.33 &  1.50 &   626 &  1.43 &  1.58 \\
Cum. earnings ($\times 1,000)$   &   118 &  1.50 &  1.75 &   123 &  1.55 &  1.93 \\
\midrule
\textbf{25-100} & & & \\
Assets ($\times 1,000$)  &    94 &  1.38 &  1.95 &    95 &  1.38 &  1.97 \\
Hours                    &   638 &  1.51 &  1.63 &   647 &  1.24 &  2.00 \\
Cum. earnings ($\times 1,000)$   &   119 &  1.39 &  1.65 &   126 &  1.43 &  1.79 \\
\midrule
\end{tabular}


==> images/means-aggregate-ass-below-50.tex <==




\begin{tabular}[ht]{lcc}
\toprule
\multirow{2}{*}{\textbf{Initial health/Variable}} & \multicolumn{2}{c}{\textbf{Model}} \\
\cmidrule(r){2-3}
 & \textbf{Nonlinear} &  \textbf{Canonical} \\
\midrule
\textbf{All} & & \\ 
	\hspace{1em} Assets ($\times 1,000$)  &   106 &  +5.1\% \\  
	\hspace{1em} Cumulated earnings (log) &  5.53 &  +5.5\% \\  
	\hspace{1em} Employment rate          &  0.87 &  -3.6\% \\  
	\hspace{1em} Hours                    &  1749 &  +3.5\% \\  
\midrule
\textbf{Percentiles 0-10} & & \\ 
	\hspace{1em} Assets ($\times 1,000$)  &    48 & +44.1\% \\  
	\hspace{1em} Cumulated earnings (log) &  4.96 &  +5.0\% \\  
	\hspace{1em} Employment rate          &  0.73 &  +0.5\% \\  
	\hspace{1em} Hours                    &  1385 &  +5.4\% \\  
\midrule
\textbf{Percentiles 10-25} & & \\ 
	\hspace{1em} Assets ($\times 1,000$)  &    84 &  +0.6\% \\  
	\hspace{1em} Cumulated earnings (log) &  5.45 &  +5.4\% \\  
	\hspace{1em} Employment rate          &  0.88 &  -5.4\% \\  
	\hspace{1em} Hours                    &  1633 &  +3.6\% \\  
\midrule
\textbf{Percentiles 25-100} & & \\ 
	\hspace{1em} Assets ($\times 1,000$)  &   121 &  +2.1\% \\  
	\hspace{1em} Cumulated earnings (log) &  5.64 &  +5.6\% \\  
	\hspace{1em} Employment rate          &  0.89 &  -3.4\% \\  
	\hspace{1em} Hours                    &  1827 &  +3.4\% \\  
\bottomrule
\end{tabular}


==> images/means-aggregate-both.tex <==


\begin{tabular}[ht]{lcccc}
\toprule
\multirow{2}{*}{\textbf{Initial health/Variable}} & \multicolumn{2}{c}{\textbf{Nonlinear}} & \multicolumn{2}{c}{\textbf{Canonical}} \\
\cmidrule(r){2-5}
 & \textbf{All} &  \textbf{Low assets} 
 & \textbf{All} &  \textbf{Low assets} \\
\midrule
\textbf{All} & & \\ 
	\hspace{1em} Assets ($\times 1,000$)  &   164 &   106 &  +2.2\% &  +5.1\% \\  
	\hspace{1em} Cumulated earnings (log) &  5.32 &  5.53 &  +5.3\% &  +5.5\% \\  
	\hspace{1em} Employment rate          &  0.79 &  0.87 &  -6.4\% &  -3.6\% \\  
	\hspace{1em} Hours                    &  1625 &  1749 &  +4.4\% &  +3.5\% \\  
\midrule
\textbf{Percentiles 0-10} & & \\ 
	\hspace{1em} Assets ($\times 1,000$)  &    93 &    48 & +20.8\% & +44.1\% \\  
	\hspace{1em} Cumulated earnings (log) &  4.85 &  4.96 &  +4.8\% &  +5.0\% \\  
	\hspace{1em} Employment rate          &  0.70 &  0.73 &  -5.8\% &  +0.5\% \\  
	\hspace{1em} Hours                    &  1324 &  1385 &  +7.2\% &  +5.4\% \\  
\midrule
\textbf{Percentiles 10-25} & & \\ 
	\hspace{1em} Assets ($\times 1,000$)  &   137 &    84 &  +3.1\% &  +0.6\% \\  
	\hspace{1em} Cumulated earnings (log) &  5.24 &  5.45 &  +5.2\% &  +5.4\% \\  
	\hspace{1em} Employment rate          &  0.79 &  0.88 &  -8.3\% &  -5.4\% \\  
	\hspace{1em} Hours                    &  1536 &  1633 &  +5.3\% &  +3.6\% \\  
\midrule
\textbf{Percentiles 25-100} & & \\ 
	\hspace{1em} Assets ($\times 1,000$)  &   177 &   121 &  +0.9\% &  +2.1\% \\  
	\hspace{1em} Cumulated earnings (log) &  5.39 &  5.64 &  +5.4\% &  +5.6\% \\  
	\hspace{1em} Employment rate          &  0.80 &  0.89 &  -6.1\% &  -3.4\% \\  
	\hspace{1em} Hours                    &  1675 &  1827 &  +4.0\% &  +3.4\% \\  
\bottomrule
\end{tabular}


==> images/means-aggregate.tex <==
\begin{tabular}[ht]{lcc}
\toprule
\multirow{2}{*}{\textbf{Initial health/Variable}} & \multicolumn{2}{c}{\textbf{Model}} \\
\cmidrule(r){2-3}
 & \textbf{Nonlinear} &  \textbf{Canonical} \\
\midrule
\textbf{All} & & \\ 
	\hspace{1em} Assets ($\times 1,000$)  &   164 &  +2.2\% \\  
	\hspace{1em} Cumulated earnings (log) &  5.32 &  +5.3\% \\  
	\hspace{1em} Employment rate          &  0.79 &  -6.4\% \\  
	\hspace{1em} Hours                    &  1625 &  +4.4\% \\  
\midrule
\textbf{Percentiles 0-10} & & \\ 
	\hspace{1em} Assets ($\times 1,000$)  &    93 & +20.8\% \\  
	\hspace{1em} Cumulated earnings (log) &  4.85 &  +4.8\% \\  
	\hspace{1em} Employment rate          &  0.70 &  -5.8\% \\  
	\hspace{1em} Hours                    &  1324 &  +7.2\% \\  
\midrule
\textbf{Percentiles 10-25} & & \\ 
	\hspace{1em} Assets ($\times 1,000$)  &   137 &  +3.1\% \\  
	\hspace{1em} Cumulated earnings (log) &  5.24 &  +5.2\% \\  
	\hspace{1em} Employment rate          &  0.79 &  -8.3\% \\  
	\hspace{1em} Hours                    &  1536 &  +5.3\% \\  
\midrule
\textbf{Percentiles 25-100} & & \\ 
	\hspace{1em} Assets ($\times 1,000$)  &   177 &  +0.9\% \\  
	\hspace{1em} Cumulated earnings (log) &  5.39 &  +5.4\% \\  
	\hspace{1em} Employment rate          &  0.80 &  -6.1\% \\  
	\hspace{1em} Hours                    &  1675 &  +4.0\% \\  
\bottomrule
\end{tabular}


==> images/nodi_welfare_byh.tex <==
Baseline            &       -4.92&       -2.34&       -1.06&       -0.47\\
Linear              &       -5.22&       -2.38&       -1.32&       -0.44\\
Linear - reest      &       -6.53&       -2.55&       -1.38&       -0.44\\


==> images/nodi_welfare_revneu_byh.tex <==
Baseline            &        1.95&        3.73&        4.43&        4.28\\
Linear              &        1.97&        3.85&        4.56&        4.58\\
Linear - reest      &        0.74&        3.71&        4.54&        4.64\\


==> images/shockBadCVcmearn.tex <==
10                  &      -0.014&      -0.002&      -0.004&      -0.003&      -0.013&      -0.002\\
80                  &      -0.017&      -0.003&      -0.003&      -0.003&      -0.013&      -0.003\\
150                 &      -0.002&      -0.001&       0.001&      -0.001&       0.001&      -0.001\\


==> images/shockBadIQRabb-bas.tex <==
10                  &       3.560&       0.099&       0.018\\
80                  &      -0.130&       0.027&       0.016\\
150                 &      -0.227&       0.020&       0.006\\


==> images/shockBadIQRlin-bas.tex <==
10                  &       1.008&       0.068&       0.022\\
80                  &      -0.150&       0.009&       0.006\\
150                 &      -0.204&       0.026&       0.006\\


==> images/shockBadIQRlin-lcc.tex <==
10                  &       0.083&       0.034&       0.013\\
80                  &      -0.009&       0.015&       0.005\\
150                 &      -0.004&       0.012&       0.004\\


==> images/shockBadIQRlll-bas.tex <==
10                  &       1.374&       0.095&       0.033\\
80                  &      -0.137&       0.014&      -0.015\\
150                 &      -0.166&      -0.053&       0.032\\


==> images/shockBadlin-bas.tex <==
10                  &      -19870&       -5424&       -2749&      -0.595&      -0.082&      -0.031\\
80                  &      -10378&       -6685&       -3543&      -0.662&      -0.133&      -0.051\\


==> images/shockBadlll-bas.tex <==
10                  &      -21704&       -5386&       -2824&      -0.593&      -0.074&      -0.029\\
80                  &      -13593&       -8090&       -3957&      -0.618&      -0.135&      -0.052\\
150                 &        2493&      -14362&       -8719&      -0.207&      -0.178&      -0.095\\


==> images/shocktable-hinit.tex <==
\begin{tabular}[ht]{lccc}
\toprule
\multirow{2}{*}{\textbf{Initial health/Shock}} & \multicolumn{3}{c}{\textbf{Model}} \\
\cmidrule(r){2-4}
 & \textbf{Nonlinear} & \textbf{Linear} & \textbf{Canonical} \\
\midrule
\multicolumn{4}{l}{\textbf{$\tau_{init}=0.9$}} \\
\multicolumn{4}{l}{\hspace{1em}\textbf{$\tau_{shock}=0.1$}} \\
	 \hspace{1em} Assets (x1,000)    &    98 &   108 \\  
	 \hspace{1em} Earnings (x1,000)  &   322 &   329 \\  
	 \hspace{1em} \% working         &  0.87 &  0.86 \\  
	 \hspace{1em} Hours              &  1962 &  2037 \\  
\midrule
\multicolumn{4}{l}{\hspace{1em}\textbf{$\tau_{shock}=0.5$}} \\
	 \hspace{1em} Assets (x1,000)    &   107 &   118 \\  
	 \hspace{1em} Earnings (x1,000)  &   338 &   350 \\  
	 \hspace{1em} \% working         &  0.87 &  0.86 \\  
	 \hspace{1em} Hours              &  2037 &  2106 \\  
\midrule
\multicolumn{4}{l}{\hspace{1em}\textbf{$\tau_{shock}=0.9$}} \\
	 \hspace{1em} Assets (x1,000)    &   116 &   121 \\  
	 \hspace{1em} Earnings (x1,000)  &   355 &   360 \\  
	 \hspace{1em} \% working         &  0.88 &  0.87 \\  
	 \hspace{1em} Hours              &  2107 &  2138 \\  
\midrule
\bottomrule
\end{tabular}


==> images/shocktable-linit.tex <==
\begin{tabular}[ht]{lccc}
\toprule
\multirow{2}{*}{\textbf{Initial health/Shock}} & \multicolumn{3}{c}{\textbf{Model}} \\
\cmidrule(r){2-4}
 & \textbf{Nonlinear} & \textbf{Linear} & \textbf{Canonical} \\
\midrule
\multicolumn{4}{l}{\textbf{$\tau_{init}=0.1$}} \\
\multicolumn{4}{l}{\hspace{1em}\textbf{$\tau_{shock}=0.1$}} \\
	 \hspace{1em} Assets (x1,000)    &    22 &    25 \\  
	 \hspace{1em} Earnings (x1,000)  &   148 &   144 \\  
	 \hspace{1em} \% working         &  0.60 &  0.57 \\  
	 \hspace{1em} Hours              &  1357 &  1393 \\  
\midrule
\multicolumn{4}{l}{\hspace{1em}\textbf{$\tau_{shock}=0.5$}} \\
	 \hspace{1em} Assets (x1,000)    &    43 &    45 \\  
	 \hspace{1em} Earnings (x1,000)  &   217 &   201 \\  
	 \hspace{1em} \% working         &  0.78 &  0.72 \\  
	 \hspace{1em} Hours              &  1532 &  1568 \\  
\midrule
\multicolumn{4}{l}{\hspace{1em}\textbf{$\tau_{shock}=0.9$}} \\
	 \hspace{1em} Assets (x1,000)    &    60 &    61 \\  
	 \hspace{1em} Earnings (x1,000)  &   254 &   239 \\  
	 \hspace{1em} \% working         &  0.83 &  0.78 \\  
	 \hspace{1em} Hours              &  1656 &  1700 \\  
\midrule
\bottomrule
\end{tabular}


==> images/shocktable-minit.tex <==
\begin{tabular}[ht]{lccc}
\toprule
\multirow{2}{*}{\textbf{Initial health/Shock}} & \multicolumn{3}{c}{\textbf{Model}} \\
\cmidrule(r){2-4}
 & \textbf{Nonlinear} & \textbf{Linear} & \textbf{Canonical} \\
\midrule
\multicolumn{4}{l}{\textbf{$\tau_{init}=0.5$}} \\
\multicolumn{4}{l}{\hspace{1em}\textbf{$\tau_{shock}=0.1$}} \\
	 \hspace{1em} Assets (x1,000)    &    66 &    69 \\  
	 \hspace{1em} Earnings (x1,000)  &   260 &   252 \\  
	 \hspace{1em} \% working         &  0.84 &  0.79 \\  
	 \hspace{1em} Hours              &  1680 &  1747 \\  
\midrule
\multicolumn{4}{l}{\hspace{1em}\textbf{$\tau_{shock}=0.5$}} \\
	 \hspace{1em} Assets (x1,000)    &    77 &    82 \\  
	 \hspace{1em} Earnings (x1,000)  &   283 &   281 \\  
	 \hspace{1em} \% working         &  0.85 &  0.83 \\  
	 \hspace{1em} Hours              &  1772 &  1847 \\  
\midrule
\multicolumn{4}{l}{\hspace{1em}\textbf{$\tau_{shock}=0.9$}} \\
	 \hspace{1em} Assets (x1,000)    &    89 &    95 \\  
	 \hspace{1em} Earnings (x1,000)  &   304 &   307 \\  
	 \hspace{1em} \% working         &  0.86 &  0.85 \\  
	 \hspace{1em} Hours              &  1871 &  1940 \\  
\midrule
\bottomrule
\end{tabular}


==> images/tab-estimates.tex <==

\begin{tabular}{llllllc} 
  \toprule \multicolumn{2}{l}{Calibrated} & & \multicolumn{2}{l}{Estimated} &  \\ \midrule  
    Time endowment & $L$ & {4880} &      
    Consumption weight & $\gamma$  & 0.4  \\
    Consumption floor & $\underbar{c}$ & {1660} &    
    Bequest 
        & $\phi_B$                 & 0.276 \\
    Risk aversion & $\nu$ & {4}    &      
       & $K$                       & 838516 \\
    Pension annuity rate & $p_r$ & {0.0378} &    
   Cost of health 
        & $\phi_{h}(h_{50})        $ & 1662.0 \\
    Pension contribution rate & $c_w$ & {0.06} &   
        & $\phi_{h}(h_{30})        $ & 1682.9 \\
    Discount factor & $\beta$ & {0.9756}     &    
        & $\phi_{h}(h_{20})        $ & 2976.8 \\
    Interest rate  & $r$ & 0.029 & 
        & $\phi_{h}(\underline{h})$ & 2979.4 \\
         & & & 
    Cost of work 
        & $\phi_w^1$               & 2040.9 \\
     & & & 
        & $\phi_w^2$               & 30.0 \\
     & & & 
        & $\phi_w^3$               & 7.6 \\
  \bottomrule
\end{tabular}

==> images/tabledecomp10.0.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
 	 Effects removed & \multicolumn{2}{c}{Assets} & \multicolumn{2}{c}{Earnings}   
 		 & \multicolumn{2}{c}{Empl.} & \multicolumn{2}{c}{Hours} & \multicolumn{2}{l}{CEV}   \\ \midrule 
	 All (relative to baseline) & -21.1 &\% & -8.2 &\% & -16.5 &\% & -22.0 &\% & \multicolumn{1}{c}{--} & \\ 
	 Decomposition: &&&&&&&&&& \\
	 \hspace{2em}Mortality      & -1.7 & \% & -0.2 & \% & +0.1 & \% & +1.0 & \% & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Time cost      & -17.0 & & -6.5 & & -15.1 & & -21.3 & & -9.37 &  \\ 
	 \hspace{2em}Wages          & -3.8 & & -1.2 & & -0.9 & & -0.8 & & -1.35 &  \\ 
	 \hspace{2em}Time+Wages     & -20.5 & & -8.0 & & -17.5 & & -22.3 & & -10.61 &  \\ 
	 \hspace{2em}Mortality+Time & -17.5 & & -6.6 & & -14.2 & & -20.6 & & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Mortality+Wages& -5.4 & & -1.4 & & -0.9 & & +0.2 & & \multicolumn{1}{c}{--} &  \\ \bottomrule
 \end{tabular}

==> images/tabledecomp1090.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
 	 Effects removed & \multicolumn{2}{c}{Assets} & \multicolumn{2}{c}{Earnings}   
 		 & \multicolumn{2}{c}{Empl.} & \multicolumn{2}{c}{Hours} & \multicolumn{2}{l}{CEV}   \\ \midrule 
	 None (baseline)            & 164 & & 5.3 & & 0.79 & & 1625 &  & \multicolumn{1}{c}{--} & \\ \\ 
\multicolumn{10}{c}{(a) Counterfactual health: 90th percentile} \\
	 All (relative to baseline) & +17.4 &\% & +7.1 &\% & +10.0 &\% & +20.1 &\% & \multicolumn{1}{c}{--} & \\ 
	 Decomposition: &&&&&&&&&& \\
	 \hspace{2em}Mortality      & -0.1 & \% & +0.1 & \% & -0.4 & \% & -0.6 & \% & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Time cost      & +13.4 & & +5.9 & & +9.1 & & +20.8 & & +1.41 &  \\ 
	 \hspace{2em}Wages          & +2.7 & & +1.4 & & +2.5 & & -0.3 & & +0.08 &  \\ 
	 \hspace{2em}Time+Wages     & +16.6 & & +7.0 & & +10.0 & & +20.9 & & +1.54 &  \\ 
	 \hspace{2em}Mortality+Time & +14.3 & & +6.0 & & +9.0 & & +20.2 & & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Mortality+Wages& +2.6 & & +1.5 & & +2.1 & & -0.9 & & \multicolumn{1}{c}{--} &  \\ 
\\
\multicolumn{10}{c}{(b) Counterfactual health: 10th percentile} \\
	 All (relative to baseline) & -21.1 &\% & -8.2 &\% & -16.5 &\% & -22.0 &\% & \multicolumn{1}{c}{--} & \\ \bottomrule
 \end{tabular}

==> images/tabledecomp25.0.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
 	 Effects removed & \multicolumn{2}{c}{Assets} & \multicolumn{2}{c}{Earnings}   
 		 & \multicolumn{2}{c}{Empl.} & \multicolumn{2}{c}{Hours} & \multicolumn{2}{l}{CEV}   \\ \midrule 
	 All (relative to baseline) & -11.2 &\% & -1.7 &\% & +3.9 &\% & -13.1 &\% & \multicolumn{1}{c}{--} & \\ 
	 Decomposition: &&&&&&&&&& \\
	 \hspace{2em}Mortality      & -1.3 & \% & -0.0 & \% & -0.3 & \% & +0.3 & \% & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Time cost      & -9.2 & & -1.2 & & +4.8 & & -13.2 & & -5.41 &  \\ 
	 \hspace{2em}Wages          & -1.7 & & -0.4 & & +0.2 & & -0.6 & & -0.86 &  \\ 
	 \hspace{2em}Time+Wages     & -10.5 & & -1.7 & & +3.9 & & -13.4 & & -6.19 &  \\ 
	 \hspace{2em}Mortality+Time & -9.8 & & -1.2 & & +4.7 & & -12.8 & & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Mortality+Wages& -2.9 & & -0.4 & & -0.0 & & -0.3 & & \multicolumn{1}{c}{--} &  \\ \bottomrule
 \end{tabular}

==> images/tabledecomp2575.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
 	 Effects removed & \multicolumn{2}{c}{Assets} & \multicolumn{2}{c}{Income}   
 		 & \multicolumn{2}{c}{Empl.} & \multicolumn{2}{c}{Hours} & \multicolumn{2}{l}{CEV}   \\ \midrule 
	 None (baseline)            & 164 & & 242.6 & & 0.79 & & 1625 &  & \multicolumn{1}{c}{--} & \\ \\ 
\multicolumn{9}{c}{(a) Counterfactual health: 75th percentile} \\
	 All (relative to baseline) & +12.1 &\% & +21.7 &\% & +7.6 &\% & +11.4 &\% & +2.3 &\%  \\ 
	 Decomposition: &&&&&&&&&& \\
	 \hspace{2em}Mortality      & -0.3 & \% & +0.2 & \% & -0.4 & \% & -0.5 & \% & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Time cost      & +9.7 & & +17.2 & & +7.0 & & +12.1 & & -0.11 &  \\ 
	 \hspace{2em}Wages          & +1.3 & & +3.2 & & +1.9 & & -0.5 & & -0.18 &  \\ 
	 \hspace{2em}Time+Wages     & +11.4 & & +21.1 & & +7.7 & & +12.0 & & -0.22 &  \\ 
	 \hspace{2em}Mortality+Time & +10.1 & & +17.7 & & +6.9 & & +11.4 & & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Mortality+Wages& +1.1 & & +3.4 & & +1.5 & & -1.0 & & \multicolumn{1}{c}{--} &  \\ 
\\
\multicolumn{9}{c}{(c) Counterfactual health: 25th percentile} \\
	 All (relative to baseline) & -11.2 &\% & -11.4 &\% & +3.9 &\% & -13.1 &\% & -9.3 &\%  \\ \bottomrule
 \end{tabular}

==> images/tabledecomp2590.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
 	 Effects removed & \multicolumn{2}{c}{Assets} & \multicolumn{2}{c}{Earnings}   
 		 & \multicolumn{2}{c}{Empl.} & \multicolumn{2}{c}{Hours} & \multicolumn{2}{l}{CEV}   \\ \midrule 
	 None (baseline)            & 164 & & 5.3 & & 0.79 & & 1625 &  & \multicolumn{1}{c}{--} & \\ \\ 
\multicolumn{10}{c}{(a) Counterfactual health: 90th percentile} \\
	 All (relative to baseline) & +17.4 &\% & +7.1 &\% & +10.0 &\% & +20.1 &\% & \multicolumn{1}{c}{--} & \\ 
	 Decomposition: &&&&&&&&&& \\
	 \hspace{2em}Mortality      & -0.1 & \% & +0.1 & \% & -0.4 & \% & -0.6 & \% & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Time cost      & +13.4 & & +5.9 & & +9.1 & & +20.8 & & +1.41 &  \\ 
	 \hspace{2em}Wages          & +2.7 & & +1.4 & & +2.5 & & -0.3 & & +0.08 &  \\ 
	 \hspace{2em}Time+Wages     & +16.6 & & +7.0 & & +10.0 & & +20.9 & & +1.54 &  \\ 
	 \hspace{2em}Mortality+Time & +14.3 & & +6.0 & & +9.0 & & +20.2 & & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Mortality+Wages& +2.6 & & +1.5 & & +2.1 & & -0.9 & & \multicolumn{1}{c}{--} &  \\ 
\\
\multicolumn{10}{c}{(b) Counterfactual health: 25th percentile} \\
	 All (relative to baseline) & -11.2 &\% & -1.7 &\% & +3.9 &\% & -13.1 &\% & \multicolumn{1}{c}{--} & \\ \bottomrule
 \end{tabular}

==> images/tabledecomp50.0.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
 	 Effects removed & \multicolumn{2}{c}{Assets} & \multicolumn{2}{c}{Earnings}   
 		 & \multicolumn{2}{c}{Empl.} & \multicolumn{2}{c}{Hours} & \multicolumn{2}{l}{CEV}   \\ \midrule 
	 All (relative to baseline) & +1.8 &\% & +1.2 &\% & +4.9 &\% & -3.3 &\% & \multicolumn{1}{c}{--} & \\ 
	 Decomposition: &&&&&&&&&& \\
	 \hspace{2em}Mortality      & -0.7 & \% & +0.1 & \% & -0.4 & \% & -0.3 & \% & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Time cost      & +1.1 & & +0.9 & & +4.8 & & -3.0 & & -2.57 &  \\ 
	 \hspace{2em}Wages          & -0.1 & & +0.3 & & +1.2 & & -0.5 & & -0.50 &  \\ 
	 \hspace{2em}Time+Wages     & +1.7 & & +1.0 & & +5.0 & & -2.8 & & -3.05 &  \\ 
	 \hspace{2em}Mortality+Time & +1.0 & & +1.1 & & +4.8 & & -3.4 & & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Mortality+Wages& -0.7 & & +0.4 & & +0.8 & & -0.8 & & \multicolumn{1}{c}{--} &  \\ \bottomrule
 \end{tabular}

==> images/tabledecomp75.0.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
 	 Effects removed & \multicolumn{2}{c}{Assets} & \multicolumn{2}{c}{Earnings}   
 		 & \multicolumn{2}{c}{Empl.} & \multicolumn{2}{c}{Hours} & \multicolumn{2}{l}{CEV}   \\ \midrule 
	 All (relative to baseline) & +12.1 &\% & +4.8 &\% & +7.6 &\% & +11.4 &\% & \multicolumn{1}{c}{--} & \\ 
	 Decomposition: &&&&&&&&&& \\
	 \hspace{2em}Mortality      & -0.3 & \% & +0.1 & \% & -0.4 & \% & -0.5 & \% & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Time cost      & +9.7 & & +3.9 & & +7.0 & & +12.1 & & -0.11 &  \\ 
	 \hspace{2em}Wages          & +1.3 & & +0.8 & & +1.9 & & -0.5 & & -0.18 &  \\ 
	 \hspace{2em}Time+Wages     & +11.4 & & +4.6 & & +7.7 & & +12.0 & & -0.22 &  \\ 
	 \hspace{2em}Mortality+Time & +10.1 & & +4.1 & & +6.9 & & +11.4 & & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Mortality+Wages& +1.1 & & +0.9 & & +1.5 & & -1.0 & & \multicolumn{1}{c}{--} &  \\ \bottomrule
 \end{tabular}

==> images/tabledecomp90.0.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
 	 Effects removed & \multicolumn{2}{c}{Assets} & \multicolumn{2}{c}{Earnings}   
 		 & \multicolumn{2}{c}{Empl.} & \multicolumn{2}{c}{Hours} & \multicolumn{2}{l}{CEV}   \\ \midrule 
	 All (relative to baseline) & +17.4 &\% & +7.1 &\% & +10.0 &\% & +20.1 &\% & \multicolumn{1}{c}{--} & \\ 
	 Decomposition: &&&&&&&&&& \\
	 \hspace{2em}Mortality      & -0.1 & \% & +0.1 & \% & -0.4 & \% & -0.6 & \% & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Time cost      & +13.4 & & +5.9 & & +9.1 & & +20.8 & & +1.41 &  \\ 
	 \hspace{2em}Wages          & +2.7 & & +1.4 & & +2.5 & & -0.3 & & +0.08 &  \\ 
	 \hspace{2em}Time+Wages     & +16.6 & & +7.0 & & +10.0 & & +20.9 & & +1.54 &  \\ 
	 \hspace{2em}Mortality+Time & +14.3 & & +6.0 & & +9.0 & & +20.2 & & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Mortality+Wages& +2.6 & & +1.5 & & +2.1 & & -0.9 & & \multicolumn{1}{c}{--} &  \\ \bottomrule
 \end{tabular}

==> images/tabledecompall.tex <==

 \begin{tabular}{ 
		  m{0.28\linewidth} 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
		  >{\raggedleft}m{0.08\linewidth}@{}l 
 } \toprule 
 	 Effects removed & \multicolumn{2}{c}{Assets} & \multicolumn{2}{c}{Earnings}   
 		 & \multicolumn{2}{c}{Empl.} & \multicolumn{2}{c}{Hours} & \multicolumn{2}{l}{CEV}   \\ \midrule 
	 None (baseline)            & 164 & & 5.3 & & 0.79 & & 1625 &  & \multicolumn{1}{c}{--} & \\ \\ 
\multicolumn{11}{c}{(a) Counterfactual health: 90th percentile} \\
	 All (relative to baseline) & +17.4 &\% & +7.1 &\% & +10.0 &\% & +20.1 &\% & \multicolumn{1}{c}{--} & \\ 
	 Decomposition: &&&&&&&&&& \\
	 \hspace{2em}Mortality      & -0.1 & \% & +0.1 & \% & -0.4 & \% & -0.6 & \% & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Time cost      & +13.4 & & +5.9 & & +9.1 & & +20.8 & & +1.41 &  \\ 
	 \hspace{2em}Wages          & +2.7 & & +1.4 & & +2.5 & & -0.3 & & +0.08 &  \\ 
	 \hspace{2em}Time+Wages     & +16.6 & & +7.0 & & +10.0 & & +20.9 & & +1.54 &  \\ 
	 \hspace{2em}Mortality+Time & +14.3 & & +6.0 & & +9.0 & & +20.2 & & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Mortality+Wages& +2.6 & & +1.5 & & +2.1 & & -0.9 & & \multicolumn{1}{c}{--} &  \\ 
\\
\multicolumn{11}{c}{(a) Counterfactual health: 75th percentile} \\
	 All (relative to baseline) & +12.1 &\% & +4.8 &\% & +7.6 &\% & +11.4 &\% & \multicolumn{1}{c}{--} & \\ 
	 Decomposition: &&&&&&&&&& \\
	 \hspace{2em}Mortality      & -0.3 & \% & +0.1 & \% & -0.4 & \% & -0.5 & \% & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Time cost      & +9.7 & & +3.9 & & +7.0 & & +12.1 & & -0.11 &  \\ 
	 \hspace{2em}Wages          & +1.3 & & +0.8 & & +1.9 & & -0.5 & & -0.18 &  \\ 
	 \hspace{2em}Time+Wages     & +11.4 & & +4.6 & & +7.7 & & +12.0 & & -0.22 &  \\ 
	 \hspace{2em}Mortality+Time & +10.1 & & +4.1 & & +6.9 & & +11.4 & & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Mortality+Wages& +1.1 & & +0.9 & & +1.5 & & -1.0 & & \multicolumn{1}{c}{--} &  \\ 
\\
\multicolumn{11}{c}{(a) Counterfactual health: 25th percentile} \\
	 All (relative to baseline) & -11.2 &\% & -1.7 &\% & +3.9 &\% & -13.1 &\% & \multicolumn{1}{c}{--} & \\ 
	 Decomposition: &&&&&&&&&& \\
	 \hspace{2em}Mortality      & -1.3 & \% & -0.0 & \% & -0.3 & \% & +0.3 & \% & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Time cost      & -9.2 & & -1.2 & & +4.8 & & -13.2 & & -5.41 &  \\ 
	 \hspace{2em}Wages          & -1.7 & & -0.4 & & +0.2 & & -0.6 & & -0.86 &  \\ 
	 \hspace{2em}Time+Wages     & -10.5 & & -1.7 & & +3.9 & & -13.4 & & -6.19 &  \\ 
	 \hspace{2em}Mortality+Time & -9.8 & & -1.2 & & +4.7 & & -12.8 & & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Mortality+Wages& -2.9 & & -0.4 & & -0.0 & & -0.3 & & \multicolumn{1}{c}{--} &  \\ 
\\
\multicolumn{11}{c}{(a) Counterfactual health: 90th percentile - 1st decile initial health} \\
	 None (baseline)            &  92 & & 5.3 & & 0.69 & & 1317 &  & \multicolumn{1}{c}{--} & \\ \\ 
	 All (relative to baseline) & +77.3 &\% & +7.1 &\% & +31.5 &\% & +54.4 &\% & \multicolumn{1}{c}{--} & \\ 
	 Decomposition: &&&&&&&&&& \\
	 \hspace{2em}Mortality      & -0.9 & \% & +0.1 & \% & -1.2 & \% & -0.6 & \% & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Time cost      & +60.5 & & +5.9 & & +30.5 & & +54.6 & & +1.73 &  \\ 
	 \hspace{2em}Wages          & +7.5 & & +1.4 & & +10.5 & & -1.4 & & +0.10 &  \\ 
	 \hspace{2em}Time+Wages     & +75.5 & & +7.0 & & +31.5 & & +56.0 & & +1.87 &  \\ 
	 \hspace{2em}Mortality+Time & +62.5 & & +6.0 & & +30.3 & & +53.2 & & \multicolumn{1}{c}{--} &  \\ 
	 \hspace{2em}Mortality+Wages& +6.7 & & +1.5 & & +9.3 & & -2.1 & & \multicolumn{1}{c}{--} &  \\ \bottomrule
 \end{tabular}

==> images/welfareshocksL_10_11.tex <==
Baseline            &      -0.050&       0.019&       0.094\\
Linear              &      -0.032&       0.029&       0.086\\
Linear shocks       &      -0.018&       0.007&       0.032\\
\linreest           &      -0.038&       0.033&       0.104\\


==> images/welfareshocksL_10_21.tex <==
Baseline            &      -0.006&       0.023&       0.056\\
Linear              &       0.006&       0.034&       0.065\\
Linear shocks       &      -0.015&       0.010&       0.038\\
\linreest           &       0.006&       0.037&       0.073\\


==> images/welfareshocksL_80_11.tex <==
Baseline            &      -0.117&      -0.015&       0.059\\
Linear              &      -0.115&       0.000&       0.055\\
Linear shocks       &      -0.025&       0.006&       0.031\\
\linreest           &      -0.149&      -0.003&       0.069\\


==> images/welfareshocksL_nodi_10_11.tex <==
Baseline            &      -0.008&       0.071&       0.178\\
Linear              &       0.047&       0.084&       0.134\\
\linreest           &       0.059&       0.096&       0.151\\


==> images/welfareshocksL_nodi_10_21.tex <==
Baseline            &      -0.003&       0.027&       0.066\\
Linear              &       0.011&       0.040&       0.075\\
\linreest           &       0.012&       0.043&       0.081\\


==> images/welfareshocksL_nodi_80_11.tex <==
Baseline            &      -0.013&       0.056&       0.168\\
Linear              &       0.031&       0.068&       0.130\\
\linreest           &       0.034&       0.078&       0.160\\


==> images/welfareshocksZ_10_11.tex <==
Baseline            &       -1035&         -14&         925&        -738&         221&        1271&        -415&         511&        1847\\
Linear              &        -483&         181&         782&        -483&         283&        1237&        -282&         605&        1691\\
Linear shocks       &        -216&          76&         352&        -340&         108&         514&        -306&         136&         648\\


==> images/welfareshocksZ_10_21.tex <==
Baseline            &        -147&         361&         947&         -82&         455&        1060&         -83&         445&        1096\\
Linear              &          15&         487&        1078&         115&         643&        1256&         143&         665&        1297\\
Linear shocks       &        -242&         147&         617&        -252&         193&         726&        -293&         193&         755\\


==> images/welfareshocksZ_80_11.tex <==
Baseline            &       -1676&        -283&         535&       -1624&        -433&         664&       -1345&         -80&        1238\\
Linear              &       -1334&           1&         450&       -1713&        -303&         659&       -1460&          84&        1198\\
Linear shocks       &        -300&          61&         330&        -462&          73&         514&        -449&         113&         636\\


==> images/welfareshocks_10_11.tex <==
Baseline            &        -669&         284&        1492\\
Linear              &        -391&         367&        1387\\
Linear shocks       &        -280&         107&         531\\


==> images/welfareshocks_10_21.tex <==
Baseline            &        -100&         421&        1047\\
Linear              &          97&         609&        1228\\
Linear shocks       &        -268&         178&         710\\


==> images/welfareshocks_80_11.tex <==
Baseline            &       -1504&        -207&         872\\
Linear              &       -1480&           4&         822\\
Linear shocks       &        -403&          86&         513\\


==> images/welfareshocks_nodi_10_11.tex <==
Baseline            &        -143&        1351&        3356\\
Linear              &         853&        1510&        2589\\
Linear shocks       &        -283&         206&         779\\


==> images/welfareshocks_nodi_10_21.tex <==
Baseline            &         -51&         511&        1254\\
Linear              &         207&         731&        1413\\
Linear shocks       &        -290&         209&         806\\


==> images/welfareshocks_nodi_80_11.tex <==
Baseline            &        -226&         928&        2774\\
Linear              &         483&        1102&        2272\\
Linear shocks       &        -277&         163&         684\\

